CDLNet: Noise-Adaptive Convolutional Dictionary Learning Network for Blind Denoising and Demosaicing

Deep learning based methods hold state-of-the-art results in low-level image processing tasks, but remain difficult to interpret due to their black-box construction. Unrolled optimization networks present an interpretable alternative to constructing deep neural networks by deriving their architecture from classical iterative optimization methods without use of tricks from the standard deep learning tool-box. So far, such methods have demonstrated performance close to that of state-of-the-art models while using their interpretable construction to achieve a comparably low learned parameter count. In this work, we propose an unrolled convolutional dictionary learning network (CDLNet) and demonstrate its competitive denoising and joint denoising and demosaicing (JDD) performance both in low and high parameter count regimes. Specifically, we show that the proposed model outperforms state-of-the-art fully convolutional denoising and JDD models when scaled to a similar parameter count. In addition, we leverage the model's interpretable construction to propose a noise-adaptive parameterization of thresholds in the network that enables state-of-the-art blind denoising performance, and near perfect generalization on noise-levels unseen during training. Furthermore, we show that such performance extends to the JDD task and unsupervised learning.

==> CDLNet _OJSP_CameraReadyArxiv/scrap.tex <==
% \IEEEPARstart{I}{n} 
% recent years, deep-learning methods have become \soa in imaging inverse
% problems such as denoising \cite{DnCNN,FFDNet}, compressed-sensing \cite{Lecouat2020Games},
% super-resolution \cite{DnCNN}, and more. However, these deep neural
% networks (DNN) and their building blocks are currently not well understood, making it ineffective to draw on knowledge from
% decades of signal processing and optimization research for insight or
% improvement. As a result, poorly understood tools such as
% batch-normalization \cite{Ioffe2015}, residual-learning, and feature-domain processing, have become staples for deep-learning
% architectures. So called ``unrolled optimization" DNNs \cite{unrolling} propose a promising avenue to remedy this by deriving their network architecture from $K$ iterations of an iterative optimization algorithm. Existing unrolled optimization DNNs are able to achieve \soa results on image restoration tasks without the use of the previously mentioned standard deep-learning toolbox  \cite{Simon2019, Lecouat2020Games}. However, these formulations mostly leverage their interpretability to reduce network parameter count in comparison to popular DNNs. In this work, we present a further desirable quality to be gained from interpretable model construction: \textit{robustness}. 

% Our proposed method tackles natural-image denoising via unrolled convolutional dictionary learning (CDL), which we call CDLNet. The convolutional dictionary learning model is rooted in the sparse representation prior, where we assume our signals $\x \in \R^N$ may be represented by a linear combination of only a few vectors (atoms) from a larger dictionary, $\bm{D}$,
% %
% \begin{equation} \label{eqn:sparse_rep}
% \exists ~ \z ~ \mathrm{s.t.} \quad \x = \bm{D}\z, \quad \norm{\z}_0 \ll N,
% \end{equation}
% %
% where $\norm{\z}_0 \coloneqq \abs{\{i : \z[i] \neq 0 \}}$ is the $\ell_0$ pseudo-norm (a.k.a counting norm). With some assumptions on the level of sparsity in $\z$ and diversity (incoherence) of the dictionary atoms, stable and unique recovery of $\z$ from $\x$ may be guaranteed \cite{Mallat}. A primary focus of signal processing literature in the last decade and a half has been on the selection of a representation dictionary, in which learning based methods such as KSVD \cite{KSVD} brought \soa performance in image restoration tasks. Given a data-set $\mathcal{X}=\{\x_i\}$, the dictionary learning problem may be formulated with an $\ell_1$-norm relaxation of the $\ell_0$ pseudo-norm, which has been shown to promote sparsity,
% %
% \begin{equation} \label{eqn:dict_learn}
% \underset{\bm{D}\in \mathcal{C}, \{\z_i\}}{\mathrm{minimize}} ~  \sum_{\x_i\in\mathcal{X}} \frac{1}{2}\norm{\bm{D}\z_i -
% \x_i}_2^2 + \lambda \norm{\z_i}_1.
% \end{equation}
% %
% The regularization parameter $\lambda$ gives a data-fidelity vs. sparsity trade-off, and $\bm{D}$ is restricted to the constraint set of columns in the unit-ball,
% \begin{equation} \label{eqn:constraint}
% \mathcal{C} = \{\bm{D} : \norm{\bm{d}^m}^2 \leq 1 \, \forall m\in\{1,\cdots,M\}\},
% \end{equation}
% to prevent arbitrary scaling of coefficients.
% This formulation is amenable to the denoising problem, $\y = \x + \bnu$, by replacing the data fidelity term with in (\ref{eqn:dict_learn}) with $\norm{\bm{D}\z_i - \y_i}_2^2$. In this work, we consider the denoising problem with additive white Gaussian noise
% (AWGN), where $\bnu \sim \mathcal{N}(0,\sigma^2\bm{I})$.

% The problem in (\ref{eqn:dict_learn}) is non-convex and thus commonly solved via a Gauss-Seidel split, alternating between sparse-coding with a fixed dictionary, and updating the dictionary given sparse codes \cite{KSVD}. The iterative soft thresholding algorithm (ISTA) is one such sparse-coding algorithm, whose iterates are defined as,
% %
% \begin{equation} \label{eqn:ista}
% \z^{(k+1)} \coloneqq \ST\left(\z^{(k)} - 
% \eta^{(k)}\bm{D}^\top(\bm{D}\z^{(k)} - \y),\, \eta^{(k)}\lambda \right),
% \end{equation}
% %
% where $\ST(\x,\tau)[i] \coloneqq \sign(\x[i])\max(0, \abs{\x[i]} - \tau)$ is the element-wise soft-thresholding operator with threshold $\tau \geq 0$, $\eta^{(k)}$ is a step-size parameter, and $\lambda$ is the sparsity penalty from (\ref{eqn:dict_learn}). In the case of a convolutional dictionary, we use $M$ filters $\bm{d}^m\in \R^{P}$ whose integer translates form the columns of $\bm{D}$. The application of the dictionary (synthesis convolution) is given by 
% $\bm{D}\z = \sum_{m=1}^M \bm{d}^m \ast \z^m$, where $\z^m$ is the $m$-th channel of $\z$. 
% The corresponding analysis convolution is defined channel-wise by $(\bm{D}^\top \x)^m = \overline{\bm{d}^m} \ast \x$ where $\overline{\bm{d}^m}$ denotes the reversal of the filter. In the case of images we have $\x \in \R^{\sqrt{N}\times\sqrt{N}\times C}$ where $C$=1 for gray-scale images and $C$=3 for colored images. Consequently, for images we consider square filters $\bm{d}^m \in \R^{\sqrt{P}\times\sqrt{P}\times C}$. 

% Making a connection between ISTA and DNNs is tempting due to their iterative use of linear operators followed by point-wise non-linearities. Our work builds off the seminal work of \cite{Gregor2010} by employing a learned ISTA encoder followed by a linear synthesis dictionary.

% \subsection{Contribution of this study}
% \label{sec:Contribution}
% Points that we want to emphasize:
% \begin{itemize}
%     \item interpretable model construction:
%     \item finding a model construction based on unrolled optimization
%     \item effective convolutional model using proper initialization and pre-processing (compared to Elad and Miral that are patch based)
%     \item effect of stride from a computational perspective.
%     \item using interpretability to propose noise adaptive thresholds
%     \item application of the proposed method for denoising and demosaicing 
% \end{itemize}



% \subsection{Notation} 
% For a matrix $X\in \mathbb{R}^{m\times n}$,

==> CDLNet _OJSP_CameraReadyArxiv/shared.tex <==

% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
% \usepackage{subfigure}
% \usepackage{subcaption}
\usepackage{pgfplots}

\usepackage{multicol}
\usepackage{multirow}
\usepackage{colortbl}
\usepackage{bm}

\usepackage{url}
\usepackage{cite}
\usepackage[hidelinks]{hyperref}
\hypersetup{
    colorlinks=true,
    linkcolor=black,
    filecolor=black, 
    citecolor=black,
    urlcolor=black,
}

\ifCLASSOPTIONcompsoc
    \usepackage[caption=false, font=normalsize, labelfont=sf, textfont=sf]{subfig}
\else
\usepackage[caption=false, font=footnotesize]{subfig}
\fi
\usepackage[export]{adjustbox}

\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi


% Packages
\usepackage{amsopn}
\usepackage{mathtools}


%%%%% algorithmic 
\usepackage[algo2e,ruled,vlined,linesnumbered]{algorithm2e}
\SetInd{0em}{0.5em}
\SetKwComment{Comment}{/\!\!/}{}

%% Tikz ops
\usepgflibrary{shapes.geometric}
\usetikzlibrary{calc}
\pgfplotsset{compat=1.16}

% Tex Ops
\def\Fig{Fig.~}

% commands
\newcommand{\soa}{state-of-the-art }

\newcommand{\C}{\mathbb C}  % blackboard bold , for ``complex,'' etc
\newcommand{\R}{\mathbb R}  % reals
\newcommand{\Z}{\mathbb Z}  % integers
\newcommand{\N}{\mathcal N} % normal distribution
%\newcommand{\D}{\mathcal D} % dictionary
\newcommand{\E}{\mathbb E}  % expectation

% Operators
% for paired-delimiters:
% 	- standard brackets: \norm{arg}
% 	- scaled brackets  : \norm*{arg}
% 	- manually scaled  : \norm[\big]{arg} etc.
\DeclarePairedDelimiterX{\norm}[1]{\lVert}{\rVert}{#1} 
\DeclarePairedDelimiterX{\abs}[1]{\lvert}{\rvert}{#1}
\DeclarePairedDelimiterX{\ip}[2]{\langle}{\rangle}{#1, #2}
\DeclarePairedDelimiterX{\pfrac}[2]{(}{)}{\frac{#1}{#2}}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator*{\argmin}{arg\,min\,} % the * places underscore arg below
\DeclareMathOperator*{\argmax}{arg\,max\,}
\DeclareMathOperator{\relu}{relu}
\DeclareMathOperator{\prox}{\mathbf{prox}} % proximal operator
\DeclareMathOperator{\ST}{\mathrm{ST}} % soft-thresholding
\DeclareMathOperator{\tr}{\mathbf{tr}} % trace
\DeclareMathOperator{\rank}{\mathbf{rank}} % rank
\DeclareMathOperator{\diag}{\mathbf{diag}} % diagonal
\DeclareMathOperator{\conv}{\mathbf{conv}} % convex hull
\DeclareMathOperator{\Var}{\mathrm{Var}}   % variance
\DeclareMathOperator{\divrg}{div}
\let\vec\undefined
\DeclareMathOperator{\vec}{\mathbf{vec}} % vectorization (flattening)

\let\pderiv\undefined
\newcommand{\pderiv}[2]{\frac{\partial #1}{\partial #2}} % partial derivative
\let\deriv\undefined
\newcommand{\deriv}[2]{\frac{d\, #1}{d\, #2}} % derivative
\let\st\undefined
\newcommand{\st}{\mathrm{s.t.}} % such that

\let\D\undefined
\newcommand{\D}{\bm{D}}
\let\x\undefined
\newcommand{\x}{\bm{x}}
\let\y\undefined
\newcommand{\y}{\bm{y}}
\let\z\undefined
\newcommand{\z}{\bm{z}}
\let\n\undefined
\newcommand{\n}{\bm{n}}
\let\bnu\undefined
\newcommand{\bnu}{\bm{\nu}}

\let\w\undefined
\newcommand{\w}{\bm{w}}
\let\m\undefined
\newcommand{\m}{\bm{m}}
\let\M\undefined
\newcommand{\M}{\bm{M}}
\let\W\undefined
\newcommand{\W}{\bm{W}}

\newcommand{\secref}[1]{\S\ref{sec:#1}} % section reference with symbol


==> scrap.tex <==
% \IEEEPARstart{I}{n} 
% recent years, deep-learning methods have become \soa in imaging inverse
% problems such as denoising \cite{DnCNN,FFDNet}, compressed-sensing \cite{Lecouat2020Games},
% super-resolution \cite{DnCNN}, and more. However, these deep neural
% networks (DNN) and their building blocks are currently not well understood, making it ineffective to draw on knowledge from
% decades of signal processing and optimization research for insight or
% improvement. As a result, poorly understood tools such as
% batch-normalization \cite{Ioffe2015}, residual-learning, and feature-domain processing, have become staples for deep-learning
% architectures. So called ``unrolled optimization" DNNs \cite{unrolling} propose a promising avenue to remedy this by deriving their network architecture from $K$ iterations of an iterative optimization algorithm. Existing unrolled optimization DNNs are able to achieve \soa results on image restoration tasks without the use of the previously mentioned standard deep-learning toolbox  \cite{Simon2019, Lecouat2020Games}. However, these formulations mostly leverage their interpretability to reduce network parameter count in comparison to popular DNNs. In this work, we present a further desirable quality to be gained from interpretable model construction: \textit{robustness}. 

% Our proposed method tackles natural-image denoising via unrolled convolutional dictionary learning (CDL), which we call CDLNet. The convolutional dictionary learning model is rooted in the sparse representation prior, where we assume our signals $\x \in \R^N$ may be represented by a linear combination of only a few vectors (atoms) from a larger dictionary, $\bm{D}$,
% %
% \begin{equation} \label{eqn:sparse_rep}
% \exists ~ \z ~ \mathrm{s.t.} \quad \x = \bm{D}\z, \quad \norm{\z}_0 \ll N,
% \end{equation}
% %
% where $\norm{\z}_0 \coloneqq \abs{\{i : \z[i] \neq 0 \}}$ is the $\ell_0$ pseudo-norm (a.k.a counting norm). With some assumptions on the level of sparsity in $\z$ and diversity (incoherence) of the dictionary atoms, stable and unique recovery of $\z$ from $\x$ may be guaranteed \cite{Mallat}. A primary focus of signal processing literature in the last decade and a half has been on the selection of a representation dictionary, in which learning based methods such as KSVD \cite{KSVD} brought \soa performance in image restoration tasks. Given a data-set $\mathcal{X}=\{\x_i\}$, the dictionary learning problem may be formulated with an $\ell_1$-norm relaxation of the $\ell_0$ pseudo-norm, which has been shown to promote sparsity,
% %
% \begin{equation} \label{eqn:dict_learn}
% \underset{\bm{D}\in \mathcal{C}, \{\z_i\}}{\mathrm{minimize}} ~  \sum_{\x_i\in\mathcal{X}} \frac{1}{2}\norm{\bm{D}\z_i -
% \x_i}_2^2 + \lambda \norm{\z_i}_1.
% \end{equation}
% %
% The regularization parameter $\lambda$ gives a data-fidelity vs. sparsity trade-off, and $\bm{D}$ is restricted to the constraint set of columns in the unit-ball,
% \begin{equation} \label{eqn:constraint}
% \mathcal{C} = \{\bm{D} : \norm{\bm{d}^m}^2 \leq 1 \, \forall m\in\{1,\cdots,M\}\},
% \end{equation}
% to prevent arbitrary scaling of coefficients.
% This formulation is amenable to the denoising problem, $\y = \x + \bnu$, by replacing the data fidelity term with in (\ref{eqn:dict_learn}) with $\norm{\bm{D}\z_i - \y_i}_2^2$. In this work, we consider the denoising problem with additive white Gaussian noise
% (AWGN), where $\bnu \sim \mathcal{N}(0,\sigma^2\bm{I})$.

% The problem in (\ref{eqn:dict_learn}) is non-convex and thus commonly solved via a Gauss-Seidel split, alternating between sparse-coding with a fixed dictionary, and updating the dictionary given sparse codes \cite{KSVD}. The iterative soft thresholding algorithm (ISTA) is one such sparse-coding algorithm, whose iterates are defined as,
% %
% \begin{equation} \label{eqn:ista}
% \z^{(k+1)} \coloneqq \ST\left(\z^{(k)} - 
% \eta^{(k)}\bm{D}^\top(\bm{D}\z^{(k)} - \y),\, \eta^{(k)}\lambda \right),
% \end{equation}
% %
% where $\ST(\x,\tau)[i] \coloneqq \sign(\x[i])\max(0, \abs{\x[i]} - \tau)$ is the element-wise soft-thresholding operator with threshold $\tau \geq 0$, $\eta^{(k)}$ is a step-size parameter, and $\lambda$ is the sparsity penalty from (\ref{eqn:dict_learn}). In the case of a convolutional dictionary, we use $M$ filters $\bm{d}^m\in \R^{P}$ whose integer translates form the columns of $\bm{D}$. The application of the dictionary (synthesis convolution) is given by 
% $\bm{D}\z = \sum_{m=1}^M \bm{d}^m \ast \z^m$, where $\z^m$ is the $m$-th channel of $\z$. 
% The corresponding analysis convolution is defined channel-wise by $(\bm{D}^\top \x)^m = \overline{\bm{d}^m} \ast \x$ where $\overline{\bm{d}^m}$ denotes the reversal of the filter. In the case of images we have $\x \in \R^{\sqrt{N}\times\sqrt{N}\times C}$ where $C$=1 for gray-scale images and $C$=3 for colored images. Consequently, for images we consider square filters $\bm{d}^m \in \R^{\sqrt{P}\times\sqrt{P}\times C}$. 

% Making a connection between ISTA and DNNs is tempting due to their iterative use of linear operators followed by point-wise non-linearities. Our work builds off the seminal work of \cite{Gregor2010} by employing a learned ISTA encoder followed by a linear synthesis dictionary.

% \subsection{Contribution of this study}
% \label{sec:Contribution}
% Points that we want to emphasize:
% \begin{itemize}
%     \item interpretable model construction:
%     \item finding a model construction based on unrolled optimization
%     \item effective convolutional model using proper initialization and pre-processing (compared to Elad and Miral that are patch based)
%     \item effect of stride from a computational perspective.
%     \item using interpretability to propose noise adaptive thresholds
%     \item application of the proposed method for denoising and demosaicing 
% \end{itemize}



% \subsection{Notation} 
% For a matrix $X\in \mathbb{R}^{m\times n}$,
